Appearance of innermost stable circular orbits of accretion discs around rotating neutron stars

The innermost stable cicular orbit (ISCO) of an accretion disc orbiting a neutron star (NS) is often assumed a unique prediction of general relativity. However, it has been argued that ISCO also appears around highly elliptic bodies described by Newtonian theory. In this sense, the behaviour of an ISCO around a rotating oblate neutron star is formed by the interplay between relativistic and Newtonian effects. Here we briefly explore the consequences of this interplay using a straightforward analytic approach as well as numerical models that involve modern NS equations of state. We examine the ratio K between the ISCO radius and the radius of the neutron star. We find that, with growing NS spin, the ratio K first decreases, but then starts to increase. This non-monotonic behaviour of K can give rise to a neutron star spin interval in which ISCO appears for two very different ranges of NS mass. This may strongly affect the distribution of neutron stars that have an ISCO (ISCO-NS). When (all) neutron stars are distributed around a high mass M0, the ISCO-NS spin distribution is roughly the same as the spin distribution corresponding to all neutron stars. In contrast, if M0 is low, the ISCO-NS distribution can only have a peak around a high value of spin. Finally, an intermediate value of M0 can imply an ISCO-NS distribution divided into two distinct groups of slow and fast rotators. Our findings have immediate astrophysical applications. They can be used for example to distinguish between different models of high-frequency quasiperiodic oscillations observed in low-mass NS X-ray binaries.

==> txsy.afm.tex <==
StartFontMetrics 2.0
FontName txsy
FullName txsy
FamilyName txsy
Weight Medium
Notice (Version 3.0, GPL)
ItalicAngle 0
IsFixedPitch false
UnderlinePosition -100
UnderlineThickness 50
Version 3.0
EncodingScheme FontSpecific
FontBBox -22 -944 1227 866
CapHeight 720
XHeight 676
Descender -944
Ascender 677
StartCharMetrics 128
C 0 ; WX 636 ; N minus ; B 62 229 574 285 ;
C 1 ; WX 250 ; N periodcentered ; B 70 203 181 314 ;
C 2 ; WX 636 ; N multiply ; B 56 -5 580 520 ;
C 3 ; WX 471 ; N asteriskmath ; B 62 63 409 450 ;
C 4 ; WX 636 ; N divide ; B 62 0 574 514 ;
C 5 ; WX 512 ; N diamondmath ; B 42 34 470 480 ;
C 6 ; WX 636 ; N plusminus ; B 62 0 574 514 ;
C 7 ; WX 636 ; N minusplus ; B 62 0 574 514 ;
C 8 ; WX 636 ; N circleplus ; B 17 -44 619 558 ;
C 9 ; WX 636 ; N circleminus ; B 17 -44 619 558 ;
C 10 ; WX 636 ; N circlemultiply ; B 17 -44 619 558 ;
C 11 ; WX 636 ; N circledivide ; B 17 -44 619 558 ;
C 12 ; WX 636 ; N circledot ; B 17 -44 619 558 ;
C 13 ; WX 862 ; N circlecopyrt ; B 17 -156 845 670 ;
C 14 ; WX 497 ; N openbullet ; B 62 71 435 443 ;
C 15 ; WX 497 ; N bullet ; B 62 71 435 443 ;
C 16 ; WX 636 ; N equivasymptotic ; B 51 60 585 454 ;
C 17 ; WX 636 ; N equivalence ; B 62 59 574 455 ;
C 18 ; WX 636 ; N reflexsubset ; B 52 -58 584 572 ;
C 19 ; WX 636 ; N reflexsuperset ; B 52 -58 584 572 ;
C 20 ; WX 636 ; N lessequal ; B 62 -58 574 574 ;
C 21 ; WX 636 ; N greaterequal ; B 62 -58 574 574 ;
C 22 ; WX 636 ; N precedesequal ; B 62 -58 574 590 ;
C 23 ; WX 636 ; N followsequal ; B 62 -58 574 590 ;
C 24 ; WX 636 ; N similar ; B 56 177 581 337 ;
C 25 ; WX 636 ; N approxequal ; B 56 75 581 439 ;
C 26 ; WX 636 ; N propersubset ; B 52 8 584 506 ;
C 27 ; WX 636 ; N propersuperset ; B 52 8 584 506 ;
C 28 ; WX 918 ; N lessmuch ; B 52 5 866 508 ;
C 29 ; WX 918 ; N greatermuch ; B 52 5 866 508 ;
C 30 ; WX 636 ; N precedes ; B 62 -13 574 525 ;
C 31 ; WX 636 ; N follows ; B 62 -13 574 525 ;
C 32 ; WX 964 ; N arrowleft ; B 62 52 902 462 ;
C 33 ; WX 964 ; N arrowright ; B 62 52 902 462 ;
C 34 ; WX 499 ; N arrowup ; B 45 -163 454 677 ;
C 35 ; WX 499 ; N arrowdown ; B 45 -163 454 677 ;
C 36 ; WX 964 ; N arrowboth ; B 62 52 902 462 ;
C 37 ; WX 964 ; N arrownortheast ; B 62 -163 902 677 ;
C 38 ; WX 964 ; N arrowsoutheast ; B 62 -163 902 677 ;
C 39 ; WX 636 ; N similarequal ; B 62 127 574 439 ;
C 40 ; WX 964 ; N arrowdblleft ; B 62 5 902 510 ;
C 41 ; WX 964 ; N arrowdblright ; B 62 5 902 510 ;
C 42 ; WX 550 ; N arrowdblup ; B 23 -163 527 677 ;
C 43 ; WX 550 ; N arrowdbldown ; B 23 -163 527 677 ;
C 44 ; WX 964 ; N arrowdblboth ; B 62 5 912 510 ;
C 45 ; WX 964 ; N arrownorthwest ; B 62 -163 902 677 ;
C 46 ; WX 964 ; N arrowsouthwest ; B 62 -163 902 677 ;
C 47 ; WX 636 ; N proportional ; B 28 62 609 440 ;
C 48 ; WX 347 ; N prime ; B 50 45 297 470 ;
C 49 ; WX 853 ; N infinity ; B 52 62 801 440 ;
C 50 ; WX 536 ; N element ; B 52 8 484 506 ;
C 51 ; WX 536 ; N owner ; B 52 8 484 506 ;
C 52 ; WX 634 ; N triangle ; B 42 0 592 548 ;
C 53 ; WX 634 ; N triangleinv ; B 42 0 592 548 ;
C 54 ; WX 0 ; N negationslash ; B 124 -162 512 676 ;
C 55 ; WX 0 ; N mapsto ; B 62 52 170 462 ;
C 56 ; WX 587 ; N universal ; B 25 -14 562 662 ;
C 57 ; WX 587 ; N existential ; B 44 0 543 662 ;
C 58 ; WX 640 ; N logicalnot ; B 62 84 578 342 ;
C 59 ; WX 500 ; N emptyset ; B 24 -28 476 689 ;
C 60 ; WX 908 ; N Rfractur ; B 58 -18 865 741 ;
C 61 ; WX 703 ; N Ifractur ; B 74 -18 611 741 ;
C 62 ; WX 712 ; N latticetop ; B 62 0 650 550 ;
C 63 ; WX 712 ; N perpendicular ; B 62 0 650 550 ;
C 64 ; WX 639 ; N aleph ; B 30 -12 609 709 ;
C 65 ; WX 870 ; N A ; B 7 -39 863 657 ;
C 66 ; WX 718 ; N B ; B 7 -22 711 684 ;
C 67 ; WX 648 ; N C ; B 7 -49 641 669 ;
C 68 ; WX 860 ; N D ; B 7 -29 853 672 ;
C 69 ; WX 622 ; N E ; B 7 -18 615 683 ;
C 70 ; WX 669 ; N F ; B 7 -66 852 705 ;
C 71 ; WX 704 ; N G ; B 7 -167 697 679 ;
C 72 ; WX 876 ; N H ; B 7 -34 967 720 ;
C 73 ; WX 650 ; N I ; B 7 -25 643 697 ;
C 74 ; WX 775 ; N J ; B -20 -149 863 678 ;
C 75 ; WX 796 ; N K ; B 7 -28 892 697 ;
C 76 ; WX 749 ; N L ; B 7 -86 742 689 ;
C 77 ; WX 1080 ; N M ; B 7 -44 1073 704 ;
C 78 ; WX 822 ; N N ; B 7 -38 911 684 ;
C 79 ; WX 703 ; N O ; B 7 -25 696 715 ;
C 80 ; WX 709 ; N P ; B 7 -37 709 678 ;
C 81 ; WX 703 ; N Q ; B 7 -56 696 715 ;
C 82 ; WX 680 ; N R ; B 7 -22 686 691 ;
C 83 ; WX 679 ; N S ; B 7 -28 672 701 ;
C 84 ; WX 678 ; N T ; B 7 -28 831 681 ;
C 85 ; WX 897 ; N U ; B 7 -32 938 694 ;
C 86 ; WX 892 ; N V ; B 7 -37 907 676 ;
C 87 ; WX 1202 ; N W ; B 7 -24 1227 697 ;
C 88 ; WX 738 ; N X ; B 7 -29 731 693 ;
C 89 ; WX 797 ; N Y ; B 7 -68 812 721 ;
C 90 ; WX 865 ; N Z ; B 7 -110 858 706 ;
C 91 ; WX 654 ; N union ; B 62 0 592 573 ;
C 92 ; WX 654 ; N intersection ; B 62 0 592 573 ;
C 93 ; WX 654 ; N unionmulti ; B 62 0 592 573 ;
C 94 ; WX 654 ; N logicaland ; B 62 0 592 556 ;
C 95 ; WX 654 ; N logicalor ; B 62 0 592 556 ;
C 96 ; WX 466 ; N turnstileleft ; B 62 0 404 514 ;
C 97 ; WX 466 ; N turnstileright ; B 62 0 404 514 ;
C 98 ; WX 371 ; N floorleft ; B 88 -163 337 677 ;
C 99 ; WX 371 ; N floorright ; B 34 -163 283 677 ;
C 100 ; WX 371 ; N ceilingleft ; B 88 -163 337 677 ;
C 101 ; WX 371 ; N ceilingright ; B 34 -163 283 677 ;
C 102 ; WX 328 ; N braceleft ; B 48 -165 280 681 ;
C 103 ; WX 328 ; N braceright ; B 48 -166 280 680 ;
C 104 ; WX 363 ; N angbracketleft ; B 50 -163 313 677 ;
C 105 ; WX 363 ; N angbracketright ; B 50 -163 313 677 ;
C 106 ; WX 200 ; N bar ; B 72 -163 128 677 ;
C 107 ; WX 400 ; N bardbl ; B 72 -163 328 677 ;
C 108 ; WX 499 ; N arrowbothv ; B 45 -173 454 687 ;
C 109 ; WX 550 ; N arrowdblbothv ; B 23 -173 527 687 ;
C 110 ; WX 441 ; N backslash ; B 62 -161 379 678 ;
C 111 ; WX 264 ; N wreathproduct ; B 54 -4 210 563 ;
C 112 ; WX 703 ; N radical ; B 60 -944 733 56 ;
C 113 ; WX 727 ; N coproduct ; B 24 0 703 662 ;
C 114 ; WX 664 ; N nabla ; B 31 0 629 676 ;
C 115 ; WX 305 ; N integral ; B 38 -86 519 866 ;
C 116 ; WX 654 ; N unionsq ; B 62 0 592 547 ;
C 117 ; WX 654 ; N intersectionsq ; B 62 0 592 547 ;
C 118 ; WX 636 ; N subsetsqequal ; B 52 -58 584 572 ;
C 119 ; WX 636 ; N supersetsqequal ; B 52 -58 584 572 ;
C 120 ; WX 500 ; N section ; B 70 -148 426 676 ;
C 121 ; WX 500 ; N dagger ; B 59 -149 442 676 ;
C 122 ; WX 500 ; N daggerdbl ; B 58 -153 442 676 ;
C 123 ; WX 453 ; N paragraph ; B -22 -154 450 662 ;
C 124 ; WX 578 ; N club ; B 42 0 536 555 ;
C 125 ; WX 531 ; N diamond ; B 42 -12 489 572 ;
C 126 ; WX 605 ; N heart ; B 42 -7 563 561 ;
C 127 ; WX 542 ; N spade ; B 42 0 500 562 ;
EndCharMetrics
EndFontMetrics

